IS-LABEL: an Independent-Set based Labeling Scheme for Point-to-Point Distance Querying on Large Graphs

We study the problem of computing shortest path or distance between two query vertices in a graph, which has numerous important applications. Quite a number of indexes have been proposed to answer such distance queries. However, all of these indexes can only process graphs of size barely up to 1 million vertices, which is rather small in view of many of the fast-growing real-world graphs today such as social networks and Web graphs. We propose an efficient index, which is a novel labeling scheme based on the independent set of a graph. We show that our method can handle graphs of size three orders of magnitude larger than those existing indexes.

==> algorithm.tex <==
%\section{Constructing $\mathbb{L}(G)$ and Labeling}

%\section{IO Efficient Algorithms}   \label{sec:algorithm}
\section{Algorithms}   \label{sec:algorithm}

%In recent years, due to the proliferation of many massive real world networks, there has been an increasing interest in algorithms that handle large graphs.

In this section, we present the algorithms for index construction (i.e., vertex hierarchy construction and vertex labeling) and query processing using the vertex labels. In recent years, due to the proliferation of many massive real world networks, there has been an increasing interest in algorithms that handle large graphs. For processing large graphs that cannot fit in main memory, I/O cost usually dominates. Thus, we propose I/O-efficient algorithms, from which the in-memory algorithms can also be easily devised. %We also note that parallel frameworks, such as MapReduce and Pregel, may not be applicable for our

For the analysis of the I/O complexity in this section, we define the following notation \cite{Aggarwal88CACM}. Let ${\it scan}(N)=\Theta(N/B)$ and ${\it sort}(N)=\Theta(\frac{N}{B}\log_{M/B} \frac{N}{B})$, where $N$ is the amount of data being read or written from/to disk, $M$ is the main memory size, and $B$ is the disk block size ($1 \ll B \le M/2$).


\subsection{Algorithm for Index Construction}  \label{ssec:algIndex}


%Assume the input graph is in the adjacency list format.
%In ${\it adj}_G (v)$, $\omega(v,u)$ for each adjacent vertex $u$ is stored, so
%that it is easy to look up the weight of each edge involving $v$.
%There are two main steps in generating the next layer in the layered network.
%The first step is to generate an independent set for the vertices at $L(i)$.
%The second step is to make sure that $G(i)$ is distance preserving.
%We first describe these two steps in the following.
%Next we describe the labeling algorithm to add labels to all vertices in
%the layered network.

Although the vertex hierarchy, except $G_k$, is not required for query processing, it is needed for vertex labeling. There are two components, $\mathbb{L}$ and $\mathbb{G}$, in the vertex hierarchy; thus, we have the following two main steps: (1) computing each independent vertex set $L_i \in \mathbb{L}$, and (2) constructing each distance-preserving graph $G_i \in \mathbb{G}$. We first describe these two steps, followed by the construction of the overall vertex hierarchy, and finally the vertex labeling.


\subsubsection{Constructing $L_i$}  \label{sssec:L_i}


%Since we want to minimize the labeling sizes, and the labeling is
%affected by the outgoing degrees of the vertices to be labeled,
%we first sort the adjacency lists in increasing degrees.
%This follows the idea in the greedy algorithm in \cite{HR94} which
%achieves a $(\triangle +2 )/3$ approximation ratio for the
%NP-hard problem of
%maximum independent set or stable set problem where the maximum degree
%of the given graph is $\triangle$. The greedy algorithm simply
%keep choosing the minimum degree vertex in the graph and remove its
%neighbors.

%There are also many polynomial-time approximation algorithms \cite{Dharwadker_06} which we can use to find a sub-optimal maximum independent set, whose size is in general greater than $\lceil n/(d+1)\rceil$ and hence can reduce more maximum independent set computations.

We want to maximize the size of each $L_i$ as this helps to minimize the number of levels $h$ and hence also minimizes the vertex label size. However, maximizing $L_i$ means computing the maximum independent set of $G_i$, which is an NP-hard problem.

%Since we want to minimize the labeling sizes, and the labeling is
%affected by the outgoing degrees of the vertices to be labeled,
%our algorithm chooses the vertices in increasing degrees and
%each time include the vertex while removing its neighbors since they will
%violate the independent set requirements.
%We first sort the adjacency lists in increasing degrees.
%Next we scan the sorted adjacency lists.
%Let ${\it adj}_{G_i}(u)$ be the next adjacency list.
%A buffer $L'$ is used to store vertices that will
%not qualify in $L_i$ due to vertex dependency.
%If $u$ is not in $L'$, we insert $u$ into $L(i)$.
%For each $v$ in ${\it adj}_{G_i}(u)$,
%if $v$ is not in $L'$, we insert $v$ into $L'$.
%We also need to record the edges in ${\it adj}_{G_i}(v)$
%for vertices $v$ added to $L_i$, they are
%stored in ${\it ADJ}(L(i))$. These will be used for the
%addition of augmenting edges for distance
%preservation.

%Since we want to minimize the label size, and the label size of a vertex is related to the degree of the vertex (higher degree

%\textbf{Since we want to minimize the labeling sizes, and the labeling is affected by the outgoing degrees of the vertices to be labeled, in what way is it affected so that we should select minimum degree vertex first?}

We adopt a greedy strategy to approximate the set of maximum independent set of $G_i$ by selecting the vertex with minimum degree at each step \cite{HalldorssonR97algorithmica}, since small degree vertices have smaller number of dependent (i.e., adjacent) vertices and hence more vertices are left as candidates for independent set at the next step. Moreover, the greedy algorithm can also be easily extended to give an I/O-efficient algorithm that handles the case when $G_i$ is too large to fit in main memory, as described in Algorithm \ref{alg:L_i}.

The algorithm computes an independent set $L_i$ of $G_i$, together with the adjacency lists of the vertices in $L_i$, denoted by ${\it ADJ}(L_i)$. We use ${\it ADJ}(L_i)$ to construct $G_{i+1}$ in Section \ref{sssec:G_i}. To compute $L_i$, we also keep those vertices that have been excluded from $L_i$ in the algorithm, as denoted by $L'$. We use a buffer to keep the current $L_i$ and ${\it ADJ}(L_i)$, and another buffer to keep $L'$.

The algorithm first makes a copy of $G_i$, let it be $G'_i$, and then sorts the adjacency lists in $G'_i$ in ascending order of the vertex degrees (i.e., the sizes of the adjacency lists). Then, we read $G'_i$ in this sorted order, i.e., the adjacency lists of vertices with smaller degrees are read first. For each ${\it adj}_{G'_i}(u)$ read, if $u$ is not in $L'$, we include $u$ into $L_i$ and add ${\it adj}_{G'_i}(u)$ to ${\it ADJ}(L_i)$. Meanwhile, we exclude all vertices in ${\it adj}_{G'_i}(u)$ from $L_i$ because of their dependence with $u$, i.e., we add these vertices to $L'$. The algorithm terminates when ${\it adj}_{G'_i}(u)$ for all $u$ in $G'_i$ are read.

If $G_i$ is very large, it is possible that $L_i$ and ${\it ADJ}(L_i)$ are too large to be kept by a memory buffer. We can simply write the current $L_i$ and ${\it ADJ}(L_i)$ in the buffer to disk, and then clear the buffer for new contents of $L_i$ and ${\it ADJ}(L_i)$. However, when the buffer for $L'$ is full, we cannot simply flush the buffer since it is possible that $\exists u \in L'$, ${\it adj}_{G'_i}(u)$ has not been read yet. To tackle this without incurring random disk accesses, we scan $G'_i$ to remove all the vertices currently in $L'$, together with their adjacency lists, from $G'_i$, because these vertices have already been excluded from $L_i$. Then, we clear the buffer for $L'$.

%If we choose to fix a degree limit for all vertices in $L_i$,
%then the scanning of the adjacency lists will be stopped at the point
%where the degree limit is exceeded.


If $G'_i$ can be resident in main memory, Lines 10-11 of Algorithm \ref{alg:L_i} are not necessary and we only need to scan $G'_i$ once. If $G'_i$ is resident on disk, it is easy to see that only sequential scans of $G'_i$ are needed and expensive random disk access is avoided.

%We also use the following standard I/O complexity notations:

Algorithm \ref{alg:L_i} takes ${\it sort}(|G_i|)$ I/Os to sort $G_i$. If $|L'| < M$, we need another ${\it scan}(|G_i|)$ I/Os to read $G_i$. Otherwise, $O(|L'|/M)*{\it scan}(|G_i|)$ I/Os are required.




%\begin{algorithm}[htbp]
%
%\SetKwInOut{input}{Input}\SetKwInOut{output}{Output}
%
%{\small
%\input{A graph $G(i)=(V_{G_i},E_{G_i},\omega_{G_i})$}
%\output{$L_i$, ${\it ADJ}(L_i)$, $G'_{i+1}$}
%\tcp{$G'_{i+1}$ is $G_{i+1}$ without augmenting edges}
%\tcp{${\it ADJ}(L_i) = \{{\it adj}_{G_i}(v) : v \in L_i\}$}
%\Begin{
%    $G'_{i+1}$ = $G_i$\;
%    Allocate buffers for $L_i$, ${\it ADJ}(L_i)$, and buffer $L'$\;
%	Sort ${\it adj}_{G_i}(v)$ in $G_i$ in increasing $deg(v)$; Scan $G_i$\;
%    %Scan the sorted lists;\\
%	\ForEach{${\it adj}_{G_i}(u)$ scanned} {
%        \If{$u \not\in L'$}{
%            insert $u$ into $L_i$;
%            insert ${\it adj}_{G_i}(u)$ into ${\it ADJ}(L_i)$\;
%            \ForEach{$v$ in ${\it adj}_{G_i}(u)$}{
%                {\bf if} $v \not\in L'$ {\bf then}
%                    insert $v$ into $L'$\;
%                }
%	   }
%    if buffer for $L_i$ or ${\it ADJ}(L_i)$ is full,
%        flush the buffer\;
%    if $L'$ is full,
%        scan $G'_{i+1}$ to remove all traces of all $v \in L'$;
%        clear $L'$\;
%    }
%}
%}
%\caption{Independent Set Extraction}
%\label{alg:IndSet}	
%\end{algorithm}

%\begin{algorithm}[!t]
%
%\SetKwInOut{input}{Input}\SetKwInOut{output}{Output}
%
%{\small
%\input{$G'_i$, ${\it ADJ}(L_{i-1})$}
%\output{$G_i$}
%    initialize $E_A = \phi$\;
%    \ForEach{pair of edges $(u,v),(u,w) \in {\it ADJ}(L_{i-1})$}{
%                insert into $E_A$ edges $(v,w)$ and $(w,v)$ with
%                $\omega(v,w) = \omega_{G_{i-1}}(u,v)+\omega_{G_{i-1}}(u,w)$\;
%            }
%    sort the edges in $E_A$ by vertex ID's\;
%    sort $G'_i$ by vertex ID's\;
%    merge $E_A$ and $G'_i$ to add/update edges in $E_A$ to $G'_i$,
%    where for $(v,w)$, $\omega(v,w) = \min( \omega_{G_i}(v,w), \omega(v,w) )$\;
%    return $G_i=G'_i$\;}
%\caption{Constructing Augmented Edges}
%\label{alg:augmentedEdges}	
%\end{algorithm}

\begin{algorithm}[!t]

\SetKwInOut{input}{Input}\SetKwInOut{output}{Output}

{\small
\input{A graph $G_i =(V_{G_i},E_{G_i},\omega_{G_i})$}
\output{$L_i$ and ${\it ADJ}(L_i) = \{{\it adj}_{G_i}(v) : v \in L_i\}$}
%\Begin{
    allocate a buffer for $L_i$ and ${\it ADJ}(L_i)$, and a buffer for $L'$\;
    $G'_i \gets G_i$\;
	sort ${\it adj}_{G'_i}(v)$ in $G'_i$ in ascending order of ${\it deg}_{G'_i}(v)$\;
    %Scan the sorted lists;\\
	\ForEach{${\it adj}_{G'_i}(u)$ read in $G'_i$} {
        \If{$u \not\in L'$}{
            insert $u$ into $L_i$, and insert ${\it adj}_{G'_i}(u)$ into ${\it ADJ}(L_i)$\;
            \ForEach{$v \in {\it adj}_{G'_i}(u)$}{
                {\bf if} $v \not\in L'$ {\bf then}
                    insert $v$ into $L'$\;
            }
        }
        {\bf if} \emph{buffer for $L_i$ and ${\it ADJ}(L_i)$ is full} {\bf then}
            flush the buffer\;
        \If{buffer for $L'$ is full}{
            scan $G'_i$ to delete all $v \in L'$ and ${\it adj}_{G'_i}(v)$, and clear $L'$\;
        }
    }
%}
}
\caption{Constructing $L_i$}
\label{alg:L_i}	
\end{algorithm}



\begin{algorithm}[!t]

\SetKwInOut{input}{Input}\SetKwInOut{output}{Output}

{\small
\input{$G_{i-1}$, $L_{i-1}$ and ${\it ADJ}(L_{i-1})$}
\output{$G_i$}

    $G_i \gets G_{i-1}$\;
    remove from $G_i$ all $v \in L_{i-1}$ and ${\it adj}_{G_{i-1}}(v)$\;
    $E_A \gets \emptyset$\;
    \ForEach{${\it adj}_{G_{i-1}}(v) \in {\it ADJ}(L_{i-1})$}{
        \ForEach{$u,w \in {\it adj}_{G_{i-1}}(v)$, where $u < w$}{
            insert into $E_A$ the edges $(u,w)$ and $(w,u)$, with $\omega_{G_i}(u,w)=\omega_{G_i}(w,u)= (\omega_{G_{i-1}}(u,v)+\omega_{G_{i-1}}(v,w))$\;
        }
    }
    sort the edges in $E_A$ by vertex ID's\;

%    scan $E_A$ and $G_i$ to add/update each edge $(u,w) \in E_A$ to/in $G_i$,
%    with the minimum of $\omega_{G_i}(u,w)$ in $E_A$ or $\omega_{G_i}(u,w)$ in $G_i$ (if $(u,w)$ already exists in $G_i$)\;

    scan $E_A$ and $G_i$ to add each edge $(u,w) \in E_A$ to $G_i$, or update $\omega_{G_i}(u,w)$ with the smaller weight if $(u,w)$ already exists in $G_i$\;


%    return $G_i=G'_i$\;

}
\caption{Constructing $G_i$}
\label{alg:G_i}	
\end{algorithm}

\subsubsection{Constructing $G_i$}  \label{sssec:G_i}

%\subsubsection{Constructing Augmenting Edges}

%After the set of independent set has been extracted from $G_{i-1}$,
%resulting in a smaller graph $G'_i$,
%a set of vertices and its adjacency list has also been collected in
%${\it ADJ}(L_{i-1})$.
%Next we consider how to create the augmenting edges to $G'_i$ in order
%to form $G_i$ that can preserve the pairwise distances.
%We give an informal intuitive reasoning here.
%For each pair of edges in ${\it ADJ}(L_{i-1})$ $(u,v),(u,w)$, we consider the
%edge $(v,w)$ which may or may not exist in $G'_i$.
%Since $(u,v)$ and $(u,w)$ along with $u$ are deleted in $G_i$, it may affect the
%shortest paths that pass through $v$ and $w$, for it is possible that
%$dist_{G_i}(v,w) > dist_G(v,w)$. Hence we add an edge $(v,w)$ to
%compensate for the loss.
%If $(v,w)$ does not exist, then we add $(v,w)$ to $G'_i$ with
%a weight $d(v,w) = \omega_{G_{i-1}}(u,v) + \omega_{G_{i-1}}(u,w)$, since this
%could be the shortest path for $(v,w)$ in $G_i$.
%If $(v,w)$ does exist, we compare the current $\omega(v,w)$
%with $d(v,w)$, whichever is smaller will be the set as the new
%weight for $(v,w)$.

%We construct $G_i$ from $L_{i-1}$ and ${\it ADJ}(L_{i-1})$, which are computed by Algorithm \ref{alg:L_i}.

After obtaining $L_{i-1}$ and ${\it ADJ}(L_{i-1})$, we use them to construct $G_i$. As shown in Algorithm \ref{alg:G_i}, we first initialize $G_i$ by removing the occurrences of all vertices in $L_{i-1}$, together with their adjacency lists, from $G_{i-1}$. However, the resultant $G_i$ may not satisfy the distance preservation property. As discussed in Section \ref{ssec:layer}, the violation to this property can be fixed by the creation of a set of augmenting edges. We create these augmenting edges from ${\it ADJ}(L_{i-1})$ as follows.

When a vertex $v \in L_{i-1}$, together with ${\it adj}_{G_{i-1}}(v)$, is removed from $G_{i-1}$ to form $G_i$, what is missing in $G_i$ is the path $\langle u,v,w \rangle$ for any $u,w \in {\it adj}_{G_{i-1}}(v)$, where $u < w$ (i.e., $u$ is ordered before $w$). Thus, to preserve the distance we only need to create the augmenting edge $(u,w)$, and symmetrically $(w,u)$ for undirected graphs, with weight $(\omega_{G_{i-1}}(u,v)+\omega_{G_{i-1}}(v,w))$.

We create all such augmenting edges in Lines 4-6 of Algorithm \ref{alg:G_i} and store them in an array $E_A$. Then, we sort the edges in $E_A$ first in ascending order of the first vertex and then of the second vertex. Then, we scan both $E_A$ and $G_i$ (already sorted in its adjacency list representation), so that each edge in $E_A$ is merged into $G_i$. If an edge in $E_A$ is already in $G_i$, then its weight updated to the smaller value of its weight recorded in $E_A$ and in $G_i$.

If main memory is not sufficient, Line 2 of Algorithm \ref{alg:G_i} uses $O(|L_{i-1}|/M)*{\it scan}(|G_{i-1}|)$ I/Os, Lines 3-6 and 8 use ${\it scan}(|G_i|)$ I/Os, and Line 7 uses ${\it sort}(|G_i|)$ I/Os, since $|E_A| < |G_i|$.




%\subsubsection{Constructing $\mathbb{L}(G)$}
\subsubsection{Constructing $(\mathbb{L},\mathbb{G})$}  \label{sssec:LG}


%Hence the overall scheme to generate the layered network is to
%start with the given $G = G_1$, and keep
%repeating the two steps of extracting independent set
%(Algorithm \ref{alg:IndSet})
%and constructing augmenting edges (Algorithm \ref{alg:augmentedEdges})
%until we reach a level $k$ where $L_k$ is an
%independent set in $G_k$.

The overall scheme to construct the vertex hierarchy, $(\mathbb{L},\mathbb{G})$, is to
start with the given $G_1=G$, and keep repeating the two steps of computing $L_i$ (Algorithm \ref{alg:L_i}) and constructing $G_i$ (Algorithm \ref{alg:G_i}) until we reach a level $k$ (see Section \ref{ssec:height} for the value of $k$).


%\begin{algorithm}[htbp]
%
%\SetKwInOut{input}{Input}\SetKwInOut{output}{Output}
%
%{\small
%\input{${\it ADJ}(\mathbb{L})$}
%\output{$Label(\mathbb{L})$}
%     \For{$i = 1, ..., k$}{
%         LabelInit(${\it ADJ}(L_i), Label(L_i)$)\;
%         }
%     \For{$i=k-1,...,1$}{
%         LabelUpdate($i, Label(\mathbb{L}(G))$)}
%}
%\caption{TopDownLabeling(${\it ADJ}(\mathbb{L}), Label(\mathbb{L})$)}
%\label{alg:topdownLabeling}
%\end{algorithm}
%
%\begin{algorithm}[htbp]
%
%\SetKwInOut{input}{Input}\SetKwInOut{output}{Output}
%
%{\small
%\input{${\it ADJ}(L_i)$}
%\output{$Label(L_i)$ with only labels for parents in $G_i$}
%\tcp{$Label(L_i) = \{ (v,Label(v)): v \in L_i \}$}
%     \ForEach{$v \in L_i$}
%     {$Label(L_i)$ $\leftarrow Label(L_i) \cup \{(v,\{(v,0)\})\}$ }
%            \ForEach{${\it adj}_{G_i}(v) \in {\it ADJ}(L_i)$}{
%                \If{ $u \in {\it adj}_{G_i}(v)$ }{
%                     insert $(u, \omega_{G_i}(v,u))$ to $Label(v)$\;
%                     }
%                }
%}
%\caption{LabelInit(${\it ADJ}(L_i), Label(L_i)$)}
%\label{alg:labeling2}
%\end{algorithm}
%
%\begin{algorithm}[htbp]
%
%\SetKwInOut{input}{Input}\SetKwInOut{output}{Output}
%
%{\small
%%\input{$Label(L(i))$,...,$Label(L(1))$}
%\output{updated $Label(L_i)$}
%%\tcp{$Label(L(i)) = \{ (v,Label(v)): v \in L(i) \}$}
%    Allocate buffer $B_L$ for $Label(L_i)$\;
%    Allocate buffer $B_U$ for $Label(L_{i+1},...,Label(L_k))$\;
%	\ForEach{block $B_{L}$}{
%        \ForEach{block $B_U$}{
%            \ForEach{$(v,Label(v)) \in B_L$}{
%                \ForEach{$(u,Label(u)) \in B_U$}{
%                    \If{ $(u,d(v,u)) \in Label(v)$ }{
%                        \ForEach{$(w,d(u,w)) \in Label(u)$}{
%                            \If{ $(w,d(v,w)) \not\in Label(v)$}{
%                              $d(v,w) = \infty$\;
%                              insert $(w,d(v,w))$ to $Label(v)$}
%                            $d(v,w) = \min( d(v,w), d(v,u)+d(u,w) )$ \;
%                        }
%                    }
%                }
%            }
%        }
%    }
%}
%\caption{LabelUpdate($i,Label(\mathbb{L})$)}
%\label{alg:labeling3}
%\end{algorithm}

\begin{algorithm}[!t]

\SetKwInOut{input}{Input}\SetKwInOut{output}{Output}

{\small
\input{$(\mathbb{L},\mathbb{G})$}
\output{${\it label}(v)$, $\forall v \in V_G$}

\tcp{Initialization of vertex labels}
     \For{$i = 1, ..., k-1$}{
          \ForEach{$v \in L_i$}{
%         InitializeLabel($L_i, G_i$)\;
        ${\it label}(v) \gets \{(v,0)\} \cup \{(u, \omega_{G_i}(v,u)): u \in {\it adj}_{G_i}(v)\}$\;
     }
      }
     $\forall v \in V_{G_k}$: \ \ ${\it label}(v) \gets \{(v,0)\}$\;



\BlankLine
\BlankLine

\tcp{Top-down vertex labeling}

     \For{$i=k-1,...,1$}{
%         TopdownLabeling($i$)\;

    allocate buffer $B_L$ and load ${\it label}(v)$, for each $v \in L_i$, in $B_L$\;
    allocate buffer $B_U$ and load ${\it label}(v)$, for each $v \in L_j$ for $i < j < k$ and for each $v \in V_{G_k}$, in $B_U$\;
	\ForEach{block $B_{L}$}{
        \ForEach{block $B_U$}{
            \ForEach{${\it label}(v)$ in $B_L$}{
                \ForEach{${\it label}(u)$ in $B_U$}{
                    \If{ $(u,d(v,u)) \in {\it label}(v)$ }{
                        \ForEach{$(w,d(u,w)) \in {\it label}(u)$}{
                            \If{ $(w,d(v,w)) \not\in {\it label}(v)$}{
                                add $(w,d(v,u)+d(u,w))$ to ${\it label}(v)$\;
%                                ${\it label}(v) \gets {\it label}(v) \cup \{(w,d(v,u)+d(u,w))\}$\;
                            }
                            \Else{
                                $d(v,w) = \min( d(v,w), d(v,u)+d(u,w) )$\;
                            }
                        }
                    }
                }
            }
        }
    }

     }
}
\caption{Top-Down Vertex Labeling}
\label{alg:topdown}
\end{algorithm}

%\begin{procedure}[!t]
%
%{\small
%     \ForEach{$v \in L_i$}{
%        ${\it label}(v) \gets \{(v,0)\}$\;
%
%        \ForEach{$u \in {\it adj}_{G_i}(v)$}{
%            ${\it label}(v) \gets {\it label}(v) \cup \{(u, \omega_{G_i}(v,u))\}$\;
%        }
%     }
%}
%\caption{InitializeLabel($L_i, G_i$)}
%\label{pro:topdown1}
%\end{procedure}

%\begin{algorithm}[!t]
%
%
%{\small
%
%    allocate buffer $B_L$ and load ${\it label}(v)$, for each $v \in L_i$, in $B_L$\;
%    allocate buffer $B_U$ and load ${\it label}(v)$, for each $v \in L_j$ for $i < j < k$ and for each $v \in V_{G_k}$, in $B_U$\;
%	\ForEach{block $B_{L}$}{
%        \ForEach{block $B_U$}{
%            \ForEach{${\it label}(v)$ in $B_L$}{
%                \ForEach{${\it label}(u)$ in $B_U$}{
%                    \If{ $(u,d(v,u)) \in {\it label}(v)$ }{
%                        \ForEach{$(w,d(u,w)) \in {\it label}(u)$}{
%                            \If{ $(w,d(v,w)) \not\in {\it label}(v)$}{
%                                add $(w,d(v,u)+d(u,w))$ to ${\it label}(v)$\;
%%                                ${\it label}(v) \gets {\it label}(v) \cup \{(w,d(v,u)+d(u,w))\}$\;
%                            }
%                            \Else{
%                                $d(v,w) = \min( d(v,w), d(v,u)+d(u,w) )$\;
%                            }
%                        }
%                    }
%                }
%            }
%        }
%    }
%}
%\caption{TopdownLabeling($i$)}
%\label{alg:topdown2}
%\end{algorithm}

\subsubsection{Top-Down Vertex Labeling}    \label{sssec:topdown}



%In the design of an IO efficient algorithm for the labeling scheme,
%we first note from Corollary (\ref{cor2}) that the
%vertices in ${\it label}(v)$ will be inherited by all its descendants.
%Hence in order to compute ${\it label}(u)$, we
%can save much computation if we can simply adopt the labels of its
%ancestors. This leads to a top-down approach.
%We start from the top level of the labeling hierarchy
%and go downwards in the generation of labels.
%In the top-down mechanism, there are two phases.
%The first phase is to initialize for
%each level $i$, all labels ${\it label}(u)$, $u \in L_i$, by only creating
%entries of the form $(v,d(u,v))$ where $v$ is a parent of $u$
%in $G_i$. See Algorithm \ref{alg:labeling2}.
%We scan the adjacency list
%for all vertices $v$ in $L_i$, and enter for each neighbor an entry
%in ${\it label}(v)$.
%The second phase is to go from top level to bottom level where
%each time we deal with labels ${\it label}(v)$ for $v$ at a
%certain level $L_i$, we inherit higher level labels of ${\it label}(u)$, where
%$u \in \{L_{i+1},..., L_k\}$.
%For IO efficiency we make use of a block nested loop join
%technique for the second phase (see Algorithm \ref{alg:labeling3}).

%Definition \ref{de:label} essentially defines a procedure for computing ${\it label}(v)$ for each $v \in V_G$. However, a careful analysis will show that such a procedure, if implemented directly as it is described, involves much redundant processing as implied by Lemma \ref{le:ancestor}. From the result of Lemma \ref{le:ancestor}, we have $\forall u \in \mathcal{V}[{\it label}(v)]$, $u$ is an ancestor of $v$ by Definition \ref{de:LABEL}. Thus, $\forall w \in \mathcal{V}[{\it label}(u)$, $w \in \mathcal{V}[{\it label}(v)$ since $w$ is then also an ancestor of $v$, which implies that ${\it label}(v)$ can be computed from ${\it label}(u)$ instead of from-scratch. From this observation, we design a more efficient top-down algorithm for vertex labeling based on the following corollary of Lemma \ref{le:ancestor}.

Definition \ref{de:label} essentially defines a procedure for computing ${\it label}(v)$ for each $v \in V_G$. However, a careful analysis will show that such a procedure, if implemented directly as it is described, involves much redundant processing as implied by the following corollary of Lemma \ref{le:ancestor}.

%Lemma \ref{le:ancestor}: For each $v \in V_G$, $\mathcal{V}[{\it label}(v)]=\mathcal{V}[{\it LABEL}(v)]$.


\begin{corollary}   \label{co:ancestor}
%Let $v \in L_i$. If $u \in {\it adj}_{G_i}(v)$, then $\mathcal{V}[{\it label}(u)] \subseteq \mathcal{V}[{\it label}(v)]$.

Given a vertex $v \in L_i$, we have $\mathcal{V}[{\it label}(v)]=\{v\} \cup (\bigcup_{u \in {\it adj}_{G_i}(v)} \mathcal{V}[{\it label}(u)])$.
\end{corollary}
\begin{proof}
By Definition \ref{de:label}, $\forall u \in {\it adj}_{G_i}(v)$, $u$ will be included into $\mathcal{V}[{\it label}(v)]$. From the result of Lemma \ref{le:ancestor}, we have $\forall u \in \mathcal{V}[{\it label}(v)]$, $u$ is an ancestor of $v$ by Definition \ref{de:LABEL}. In the same way, we have $\forall w \in \mathcal{V}[{\it label}(u)]$, $w \in \mathcal{V}[{\it label}(v)]$ since $w$ is then also an ancestor of $v$. Thus, $\forall u \in {\it adj}_{G_i}(v)$, $\mathcal{V}[{\it label}(u)] \subseteq \mathcal{V}[{\it label}(v)]$.

Next, $\forall w \in \mathcal{V}[{\it label}(v)] \backslash \{v\}$, $w \in \mathcal{V}[{\it label}(u)]$ for some $u \in {\it adj}_{G_i}(v)$ because $w$ is included into $\mathcal{V}[{\it label}(v)]$ from some $u$ by Definition \ref{de:label}, and by the same procedure $w$ will be included into $\mathcal{V}[{\it label}(u)]$ when we compute ${\it label}(u)$.
\end{proof}

Corollary \ref{co:ancestor} implies that ${\it label}(v)$ can be computed from ${\it label}(u)$, for each $u \in {\it adj}_{G_i}(v)$, instead of from scratch. Based on this, we design a more efficient top-down algorithm for vertex labeling as shown in Algorithm \ref{alg:topdown}.

The algorithm consists of two stages: initialization of vertex labels and top-down vertex labeling by block nested loop join, discussed as follows.

According to Corollary \ref{co:ancestor}, we only need to add $(v,0)$ and $(u, \omega_{G_i}(v,u))$ for all $u \in {\it adj}_{G_i}(v)$ to ${\it label}(v)$, and then derive other entries of ${\it label}(v)$ from ${\it label}(u)$ in the top-down process. For each $v \in V_{G_k}$, however, we only need to add $(v,0)$ to ${\it label}(v)$ since each $v \in V_{G_k}$ has only one ancestor, i.e., $v$ itself.

After the initialization, we compute the labels for the vertices starting from the top levels to the bottom levels, i.e., from level $(k-1)$ down to level 1. We assume that the set of labels at each level may not be able to fit in main memory and hence use block nested loop join to find the matching labels, i.e., ${\it label}(u)$ for each $u \in {\it adj}_{G_i}(v)$ when we process $v$ at level $i$. Note that if $u \in {\it adj}_{G_i}(v)$, then $(u,d(v,u)) \in {\it label}(v)$ by the initialization. Thus, as shown in Lines 11-16, we derive the entries of other ancestors of $v$ from ${\it label}(u)$ directly, which essentially follows the rule specified in Definition \ref{de:label}.


%For  labeling scheme,
%first we can use block nested-loop join to get the adjacency list for the nodes in level L(i), use {\it ADJ}(L(i)) to denote. Second, block nested-loop join on {\it ADJ}(L(i)) and L(i+1), to get labels for L(i).
%Do these two steps for i from h to 1.
%Finally, scan {\it label}(L(i)) from h to 1, update the {\it label}(L(i)) with {\it label}(L(i+1)).

%For Algorithm \ref{alg:labeling2}, the IO complexity is
%$O(Scan(|{\it ADJ}(L_i)|))$.
%For Algorithm \ref{alg:labeling3}, we have a nested loop join between
%${\it label}(L_i)$ and ${\it label}(L_{i+1}) \cup ... \cup {\it label}(L_k)$
%Let $b_1(i) = |{\it label}(L_i)|$, and $b_2(i) = |{\it label}(L_{i+1}) \cup ... \cup {\it label}(L_k)$.
%The IO complexity for the join is given by
%$b_1(i)/M * b_2(i)/B$.
%Hence for Algorithm \ref{alg:topdownLabeling}, the IO complexity
%is given by
%$\sum_{i=1}^h ( Scan(|{\it ADJ}(L_i)|) + b_1(i)/M * b_2(i)/B )$.


The complexity of the algorithm is apparently dominated by the top-down process. Let $b_L(i) = |\{{\it label}(v): v \in L_i\}|$, and $b_U(i) = |\bigcup_{i < j < k}\{{\it label}(v): v \in L_j\} \cup \{{\it label}(v): v \in V_{G_k}\}|$. The I/O complexity for the block nested loop join is given by $(b_L(i)/M) * (b_U(i)/B)$. Thus, the I/O complexity of Algorithm \ref{alg:topdown} is given by $O(\sum_{i=1}^{k-1} ((b_L(i)/M) * (b_U(i)/B)))$.

%Thus, for the first step, the IO complexity is
%$\sum_{i} |G|/M * |L(i)| / B +   |G| /B =  |G| /B +  |G|/M * |V| / B.$
%Second step:
%$\sum_{i} ( |{\it ADJ}(L(i))|/M * |L(i+1)| / B +   | {\it ADJ}(L(i)) | /B) =  |G| /B +  |G|/M * |V| / B.$
%Third step:
%$\sum_{i} Scan(Label(L(i))) < (|V| ^{2}) /B$, it should be much smaller than
%$(|V| ^{2}) /B.$
%So the total IO complexity is $O( |G| /B +  |G|/M * |V| / B + (|V| ^{2}) /B).$

%\begin{theorem}
%The top-down labeling Algorithm \ref{alg:topdownLabeling} generates
%the same labeling as Algorithm \ref{alg:labeling}.
%\end{theorem}
%
%{\small PROOF}.
%First we note that for the labeling from Algorithm \ref{alg:labeling},
%the highest layer $L_k$ consists of at most one vertex for each
%connected component of $G$.
%The initial step includes $(v,0)$ in
%the label for such a vertex so we can begin the top-down process.
%After LabelInit(), we only include labels of ancestor nodes,
%this follows Corollary \ref{cor2}.
%\done


%\subsubsection{Complexity, IO, storage, and time}

%\subsubsection{Reducing the labeling size}
%
%Edge Pruning by Triangle Inequality

\subsection{Algorithm for Query Processing}  \label{ssec:algQuery}


%\subsection{P2P Distance Querying}
%Since we assume very large data sizes, the labels will not fit in memory, and labels are stored on disk.
%Then we build a simple lookup index to retrieve all labels in $label(v)$ given vertex $v$. Within $label(v)$, the entries $(u, d(v,u))$ are sorted by the vertex
%id's of $u$. In this way the search for $label(u) \cup label(v)$ involves simple scanning of the entries in $label(u)$ and $label(v)$.
%From our experiments, most of the labels are small in sizes and involves only one IO.
%
%The CPU time for query processing comes mostly from the bi-Dijkstra search.
%For a $G=(V,E)$, a binary heap can be used and Dijkstra's algorithms runs in $O((|E| + |V|) \log |V|)$ time.

For processing large datasets, the vertex labels may not fit in main memory and are stored on disk. The entries in each ${\it label}(v)$ are stored sequentially on disk and are sorted by the vertex ID's of the ancestors of $v$. Thus, ${\it label}(s) \cap {\it label}(t)$ involves simple sequential scanning of the entries in ${\it label}(s)$ and ${\it label}(t)$. From our experiments, the vertex labels are small in size and retrieving a vertex label from disk takes only one I/O.
The CPU time for query processing comes mostly from the bi-Dijkstra search. For a graph $G=(V,E)$, a binary heap can be used and Dijkstra's algorithms runs in $O((|E| + |V|) \log |V|)$ time.



%\subsection{Permutations of layers}





==> directed.tex <==
\subsection{Directed Graphs}

If the given graph is directed, we need to modify the vertex hierarchy
construction as well as the vertex labeling. Let us use $(u,v)$ to indicate an edge from $u$ to $v$.
The concept of independent set can be applied by ignoring the directions
of edges.
However, for distance preservation, we create an augmenting
edge $(u,v)$ at $G_i$ if and only if there exist a vertex
$w$ at
$G_{i-1}$, where $w \not\in E_{G_i}$ and edges $(u,w), (w,v)$ in $E_{G_{i-1}}$, such that
the sum of weights of $(u,w)$ and $(w,v)$ is less than the
weight of any edge $(u,v)$ in $E_{G(i-)}$.
We distinguish two types of ancestors for a vertex $v$,
in-ancestors and out-ancestors.\
The definition for in-ancestors is similar to that for ancestors in undirected graph, except we only consider edges from
higher level vertices to lower level vertices.
Analogously, the definition for out-ancestors involves edges going
from lower level vertices to higher level vertices.

The labeling would need to handle two directions.
For each vertex $v$ there are two labels, $\mathcal{L}_{out}(v)$ and
$\mathcal{L}_{in}(v)$.


\begin{definition}[Vertex Label]    \label{de:LABEL}
The \textbf{in-label} of a vertex $v \in V_G$, denoted by $\mathcal{L}_{in}(v)$, is defined as $\mathcal{L}_{in}(v)=\{(u,{\it dist}_G(v,u)): u \in V_G \textrm{ is an in-ancestor of \ } v\}$.
The \textbf{out-label} of a vertex $v \in V_G$, denoted by $\mathcal{L}_{out}(v)$, is defined as $\mathcal{L}_{out}(v)=\{(u,{\it dist}_G(v,u)): u \in V_G \textrm{ is an out-ancestor of \ } v\}$.
\end{definition}

Given a P2P distance query with two input vertices, $s$ and $t$, let $\mathbb{X} =$ $\mathcal{L}_{out}(s) \cap \mathcal{L}_{in}(t)$, the query answer is given as follows.

\begin{equation}    \label{eq:query2}
{\it dist}_G(s,t) = \left\{ \begin{array}{ll}
\min_{w \in \mathbb{X}}\{ d(s,w) + d(t,w) \} & \textrm{if $\mathbb{X} \neq \emptyset$}\\
\infty & \textrm{if $\mathbb{X} = \emptyset$}
\end{array} \right.
\end{equation}
In Equation \ref{eq:query2}, we retrieve $d(s,w)$ and $d(t,w)$ for each $w \in \mathbb{X}$ from $\mathcal{L}_{out}(s)$ and $\mathcal{L}_{in}(t)$, respectively. 
The remaining conversion of our mechanisms for handling directed graphs is based on the use of this equation. We skip the details for interested of space. 

==> dynamic.tex <==
\subsection{Dynamic Updates}

We consider the cases where vertices along with their adjacency lists
are inserted or deleted in the graph.
The main task is to maintain the vertex hierarchy so that P2P queries are
correctly answered.
For insertion of a new vertex $u$, we add $u$ to $G_k$.
Next we consider each vertex $v$ in the adjacency list $adj_G(u)$.
If $v$ is in $G_k$, then we simply add the edge $(u,v)$ to $E_{G_k}$
with weight $\omega(u,v)$. Otherwise, let $v \in L_i$.
We add $(u,\omega(u,v))$ to $label(v)$.
Consider the
descendants of $v$ in the vertex hierarchy. The
descendants form a tree rooted at $v$, with the edges being the
the edges $(w_i, w_{i+1})$ in $E_{G_j}$, where $j = \ell(w_i)$
and $w_i, w_{i+1}$ are descendants of $v$.
We can traverse this tree either in a depth first manner,
so that the entry $(u, d(u,w))$ is added to or modified in $label(w)$, where $w$ is a
descendant of $v$,so that the value of $d(u,w)$ is set to or 
if needed, decreased to the accumulated distance
of $\omega(u,v) + d(v,v_1),...d(v_i,w)$, where $v, v_1, ..., w$ is a path in
the tree. The IO complexity is given by
the number of descendants of $u$.
Next consider the deletion of a vertex $u$.
If $u$ is in $G_k$ and no label contains $u$, then $u$ can simply be deleted
from the adjacent lists of all its neighbors in $G_k$.
Otherwise, we look for the descendants of $u$ and remove the entry for $u$
in each descendant. In this case, the IO complexity is
determined by the number of descendants of $u$.

\begin{lemma}
The distance query answering is correct after insertion or deletion of
a vertex.
\end{lemma}



==> pathQuery.tex <==
\section{Query variations, dynamic updates and directed graphs}

\subsection{Path Queries}


When 
an augmenting edge $(u,w)$ is created in $G_i$ with $\omega_{G_i}(u,w) = \omega_{G_{i-1}}(u,v)+\omega_{G_{i-1}}(v,w)$, we record an
intermediate vertex $v$
along with the augmenting edge. This indicates that the edge is replacing a path
$u \leadsto v \leadsto w$. Note that $(u,v)$ or $(v,w)$ 
corresponds to an edge in $G_{i-1}$,
and it in turn can be an augmenting path with its own subpaths from
lower levels of the vertex hierarchy. 
If $(u,w)$ already exists in $G_i$, and weight $\omega_{G_i}(u,w)$ is set to
$\min( \omega_{G_{i-1}}(u,w), \omega_{G_{i-1}}(u,v)+\omega_{G_{i-1}}(v,w))$
and
$\omega_{G_{i-1}}(u,w) > \omega_{G_{i-1}}(u,v)+\omega_{G_{i-1}}(v,w))$,
then again $v$ is recorded as an intermediate with edge $(u,w)$, since a path
$u \leadsto v \leadsto w$ corresponds to the weight.
In the labeling process, when we include into $label(v)$ the pair
$(w, d(v,w))$, we also attach the
intermediate vertex $u$ for $(v,w)$, if any, with the pair.
The entry becomes a triple:
$(w, d(v,w), u)$.
If there is no intermediate vertex for $(v,w)$, $u$ is set to null, the triple
becomes $(w, d(v,w), NULL)$.
Note that we only keep the graph $G_k$, hence only the intermediate vertices
for augmenting paths in this graph are maintained.

Given a path query between $s$ and $t$, if the corresponding distance query
is of Type 1, the result is determined by two label entries of $(s, d(s,w), u)$ and
$(t, d(t,w), u')$. If $u$ ($u'$) is not NULL, we form two new path queries
$(s,u)$ and $u,w)$ ( $(t,u')$ and $(u',w)$ ). We recursively form path
queries in this way until no non-NULL intermediate node is encountered. It is
straight forward to form the resulting path by linking all the intermediate vertices
in a recursive manner.
If the corresponding distance query for $s$ and $t$ is of Type 2,
there are 3 possible components that gives rise to the answer, 2 label entries
and a path in $G_k$. The subpaths for the 2 label entries are derived as the above.
The path in $G_k$ is derived by expanding any augmenting edges, taking into account the intermediate vertex. New queries are formed from the expansion and such queries will be of Type 1. The IO complexity is given by
$O(|SP_G(s,t)|)$.

\subsection{Synopsis of Shortest Paths}

The path querying process can be easily altered in
order to report a synopsis (a subset of vertices) in a shortest path, this is because we can stop anywhere during the expansion of subpaths.
Furthermore, if there are important vertices that we would like to include in our answers, we simply do not include these vertices in the vertex hierarchies so that they appear in $G_k$.  

==> related.tex <==
\section{Related Work}  \label{sec:related}

Other related work, in addition to those discussed in Section \ref{sec:challenge}.

The idea is similar to contraction hierarchy in road networks \cite{GeisbergerSSD08wea}, where the shortest path from one place to another is either localized or passing through some important junctions of highways or main streets (i.e., vertices of higher hierarchy). However, such a vertex hierarchy is not natural in a general graph and generalizing

\cite{JRXL12}, \cite{Wei10}, \cite{Xiao09}


Our independent set selection bears some resemblance to
the greedy algorithm in \cite{HalldorssonR94stoc} which
achieves a $(\triangle +2 )/3$ approximation ratio for the
NP-hard problem of
maximum independent set or stable set problem where the maximum degree
of the given graph is $\triangle$. The greedy algorithm simply
keep choosing the minimum degree vertex in the graph and remove its
neighbors.
